A Systematic Evaluation of Co-folding Model Representations for Small-Molecule Learning

Small-molecule foundation models are typically pretrained on standalone molecular data, unlike vision and language models that often benefit from cross-modal or relational supervision. Protein-ligand co-folding provides a molecular analogue of such supervision by exposing models to atom-level ligand-protein interactions, raising the question of whether co-folding models can yield strong small-molecule representations. We study this question using Boltz2, a modern co-folding model, by transferring its atom-level ligand representations to standalone small-molecule tasks. Through systematic probing and distillation, we show that Boltz2 representations match or outperform existing models on the ADMET benchmark, accelerate molecular generative modeling, and improve sample efficiency in structure-guided ligand optimization. We further find that Boltz2 representations are complementary to those learned from conventional standalone molecular supervision, including 3D conformers, bioassay labels, and quantum-chemical properties. Finally, we extend representation alignment to reinforcement learning, showing that dense representation-level supervision can complement scalar rewards in molecular discovery. These results identify protein-ligand co-folding as a promising pretraining paradigm for small-molecule representation learning and position Boltz2 as a strong, off-the-shelf molecular foundation model.

==> 1_intro.tex <==
\section{Introduction}

Large-scale representation learning has shown strong transferability across a wide range of downstream tasks, particularly in language~\citep{llama3, gpt4} and vision domains~\citep{vit, dinov2}. Foundation models with large-scale pretraining have become essential for achieving state-of-the-art performance in downstream applications, serving as powerful feature extractors~\citep{radford2021learning} for predictive tasks. Beyond predictive tasks, researchers have leveraged their representations to enhance generative modeling, including distillation into denoising models~\citep{yu2024representation} and use as latent embeddings for latent diffusion models~\citep{rae}. 

In the small-molecule domain, this paradigm has motivated foundation models that learn transferable atom-level representations for drug discovery tasks such as ADMET prediction~\citep{huang2021therapeutics}. Most existing models learn from molecules considered in isolation: each training example is a small molecule associated with molecule-level supervision such as bioassay labels and quantum-chemical properties~\citep{mendez2024mole,klaser2024minimol,kim2024quantum,zhou2023unimol,li2023knowledge,sypetkowski2024scalability}. Although these models differ in architecture and objective, they share a common design choice: the small molecule itself is the primary object of representation learning, without explicit modeling of an interacting molecular partner.

%Similarly, researchers in the small-molecule domain have explored foundation models to obtain transferable molecular representations, which is significant to solve a range of downstream tasks for drug discovery, e.g., ADMET prediction~\citep{huang2021therapeutics}. Especially, existing studies have focused on atom-level representation learning for small molecules, aiming to encode atom-level mechanisms through pretraining objectives such as masked token prediction, bioassay supervision, quantum property regression, and 3D structure prediction ~\citep{mendez2024mole,klaser2024minimol,kim2024quantum,zhou2023unimol,li2023knowledge,sypetkowski2024scalability}. Although these models differ in architecture and objective, they share a common paradigm: they learn molecular representations from molecules in isolation.

%These models differ in architecture and objective, but share a common paradigm: \textit{they learn molecular representations from standalone molecular data}. 
%However, in vision and natural language processing, strong representations are often learned by going beyond standalone data and incorporating complementary cross-modal or relational supervision \citep{radford2021learning,jia2021scaling,zhai2022lit}. The molecular domain likewise provides an analogous source of supervision through extensively accumulated high-quality inter-molecular interaction data: \textit{protein-ligand co-folding 3D structure} \citep{burley2021rcsb}, where a small molecule interacts with a protein to form a protein-ligand complex. This motivates a new question:
This is in contrast to vision and language, where strong representations often arise from supervision beyond standalone data, such as cross-modal or relational signals~\citep{radford2021learning,jia2021scaling,zhai2022lit}. We argue that the molecular domain has an analogous but underexplored source of such supervision: protein-ligand co-folding structures~\citep{burley2021rcsb}, in which a small molecule interacts with a protein at the atomic level. %in which small molecules are observed through their atom-level interactions with protein environments. 

\textcolor{blue}{
Although repurposing protein–ligand co-folding models for small-molecule representation learning is conceptually straightforward, it has not been systematically studied. This gap is important because the broader utility of co-folding models remains debated: recent studies suggest that models such as AlphaFold3 may rely heavily on MSA-derived evolutionary patterns rather than a genuine atom-level understanding of molecular interactions \citep{stahl2023protein,brotzakis2025alphafold}. Establishing this baseline therefore allows us to test whether the interaction-aware supervision learned by modern co-folding models transfers beyond their original structure-prediction objective. We therefore ask:}
%These models differ in architecture and objective, but share a common paradigm: \textit{they learn molecular representations from standalone molecular data}. However, in vision and natural language processing, models often learn stronger representations by incorporating complementary information beyond the target modality, such as image-text pairs, even when evaluated on standalone modality tasks. Analogously, molecular learning can leverage an additional source of supervision: \textit{protein-ligand co-folding 3D structure prediction}, where a small molecule interacts with a protein to form a protein-ligand complex. Then, this raises a natural question:
\begin{center}
\noindent\fcolorbox{black}{gray!15}{
\parbox{0.92\linewidth}{
\centering
\textit{Can protein-ligand co-folding models provide strong atom-level representations for standalone small-molecule tasks?}
}
}
\end{center}
We hypothesize that learning protein-ligand interactions provides richer supervision than learning from standalone molecular data alone, as it captures the atom-level mechanisms underlying interactions in bound conformations, including hydrogen bonding and electrostatic interactions. If this holds, protein-ligand complexes would constitute a new supervision source for molecular representation learning, complementary to the standalone molecular data.

% Boltz is trained on collections of protein-ligand complexes and learns atomistic representations of ligands using their bound conformations, which may encode atom-level mechanisms such as hydrogen bonding and electrostatic interactions

\input{resource/background_figure}

Timely, modern protein–ligand co-folding models have transitioned from residue-level to atom-level modeling. AlphaFold3~\citep{abramson2024accurate} and its open-weight counterpart Boltz~\citep{wohlwend2024boltz1,passaro2025boltz2} are trained on large collections of protein-ligand complexes and learns atomistic representations to predict protein-ligand complexes with full atomic detail. Although their purpose is structure prediction, we are the first to transfer their atomistic representations to standalone small-molecule tasks.

%Note that this transfer is unexplored in the current literature, as skepticism remains regarding co-folding model's broader utility. Some studies argue that AlphaFold3 rely heavily on evolutionary patterns derived from MSAs rather than a genuine atom-level understanding \citep{stahl2023protein,brotzakis2025alphafold}. %In addition, prior work has shown that AlphaFold3 depend on memorization rather than fully understanding the atom-level mechanism.


\textbf{Contribution.} In this work, we investigate the potential of co-folding model, Boltz2, as a source of representations for small-molecule tasks, bridging cutting-edge protein-centric models and atom-level representation learning for small molecules. As illustrated in \Cref{fig:boltz_as_fm}, we extract atom-level representations from Boltz2 for a given small molecule and evaluate their expressiveness across a broad range of small-molecule downstream tasks. Notably, our work is the first to show that informative molecular representations can improve molecular generation and optimization.

%We show that Boltz2 provides strong atom-level representations out of the box, beyond its original protein–ligand co-folding objective. 
Through systematic experiments, we identify four key findings that position modern co-folding model, in particular Boltz2, as a strong baseline for small-molecule foundation models.
\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
\item \textbf{Predictive transfer (\Cref{sec:admet})}: Boltz representations match or outperform specialized small molecular foundation models on the extensive TDC ADMET benchmark.
\item \textbf{Generative transfer (\Cref{sec:mol_gen}):} Boltz2 representations improve molecular generative models with representation alignment~\citep{yu2024representation}.
\item \textbf{Optimization transfer (\Cref{sec:structure_guided}):} Boltz2 representations enhance sample efficiency for designing ligands to maximize the Boltz2's binding affinity score \textcolor{blue}{using a new distillation method}. 
\item \textcolor{blue}{\textbf{Representation complementarity (\Cref{sec:ablation}):} Co-folding representations occupy a distinct representation space from models pretrained on standalone molecular data.}
\end{itemize}
%These findings suggest that the representational capacity of co-folding-based representation learning has been underexplored by the community. position modern co-folding model, Boltz2, as a strong baseline for small-molecule foundation models. 
%We also note the \textit{complementarity of Boltz2 representations} with existing foundation models trained on standalone molecular data, and the improvement in downstream performance from the \textit{use of protein context} (\Cref{sec:ablation}).
Finally, we provide actionable insights for the molecular machine learning community. First, we extend representation alignment to online reinforcement learning for molecular discovery, showing how dense signals from the reward model can be used to improve sample efficiency beyond scalar rewards alone. Second, we show that combining weakly aligned representations, e.g., Boltz2 with MolE \citep{mendez2024mole}, outperforms more strongly aligned combinations, e.g., Boltz2 with MiniMol \citep{klaser2024minimol}, suggesting a practical strategy for representation fusion. 

%Beyond empirical evaluations of Boltz2 representations, we also provide three actionable insights for the molecular machine learning community:
%\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
%\item \textbf{Co-folding as complementary pretraining.} We show that predicting 3D protein-ligand interactions provides atom-level representation complementary to existing standalone molecular representation learning.
%\item \textbf{Representation-guided molecular optimization.} We extend representation alignment to online reinforcement learning for molecular discovery, showing that dense representation-level auxiliary supervision improves sample efficiency beyond scalar rewards alone.
%\item \textbf{Complementary representation ensembling.} We show that combining representations with low alignment, e.g., Boltz2 ensembled with MolE \citep{mendez2024mole}, outperforms higher alignment combinations, e.g., Boltz2 ensembled with MiniMol \citep{klaser2024minimol}, providing a useful strategy for representation fusion.
%\end{itemize}






%Meanwhile, protein–ligand co-folding models have transitioned from residue-level to atom-level modeling. AlphaFold3~\citep{abramson2024accurate} and Boltz~\citep{wohlwend2024boltz1,passaro2025boltz2}, predict protein-ligand complexes at atomic resolution. To predict how a ligand binds to a protein, these models learn atom-level representations of ligand molecules that encode inter-molecular interactions, including hydrogen bonding, and electrostatic between protein residues and ligand atoms. Their atom-level expressiveness enables accurate modeling of binding geometry and leads to improved binding pose prediction accuracy.
%This raises a natural question:
%\begin{center}
%\noindent\fcolorbox{black}{gray!15}{
%\parbox{0.92\linewidth}{
%\centering
%\textit{Can cutting-edge protein-centric models, particularly Boltz, provide strong atom-level representations for standalone small-molecule tasks?}
%}
%}
%\end{center}


%Notably, cutting-edge protein-centric models have reached atom-level granularity. AlphaFold3~\citep{abramson2024accurate} and its open-weight counterpart Boltz~\citep{wohlwend2024boltz1,passaro2025boltz2} learn atom-level representations to predict protein-ligand complexes with full atomic detail. This raises a natural question:
%\begin{center}
%\noindent\fcolorbox{black}{gray!15}{
%\parbox{0.92\linewidth}{
%\centering
%\textit{Can cutting-edge protein-centric models, particularly Boltz, provide strong atom-level representations for standalone small-molecule tasks?}
%}
%}
%\end{center}
%If this holds, it suggests that separate pretraining pipelines for small molecules may not be strictly necessary, pointing toward a more unified molecular foundation model.

%On the one hand, the co-folding training objective used in protein-centric models such as Boltz seems promising for learning strong atom-level representations. Boltz is trained on collections of protein-ligand complexes and learns atomistic representations of ligands using their bound conformations, which may encode atom-level mechanisms such as hydrogen bonding and electrostatic interactions. While prior work shows that pretraining with 3D molecular structures yields transferable representations~\citep{zaidi2023pretraining,zhou2023unimol}, Boltz leverages richer supervision from interaction context in protein-ligand co-structures.


%On the other hand, skepticism remains regarding Boltz's broader utility. Some studies argue that protein models like Boltz rely heavily on evolutionary patterns derived from MSAs rather than a genuine atom-level understanding \citep{stahl2023protein}. In addition, \citet{masters2025investigating} has shown that predictions of AlphaFold3 depend on memorization rather than fully understanding the atom-level mechanism.




%\textbf{Contribution.} In this work, we empirically investigate the potential of Boltz as a source of representations for small-molecule tasks, \textit{bridging cutting-edge protein-centric models and atom-level representation learning for small molecules}. Additionally, for the first time, we show that foundation model representations can be leveraged to guide and accelerate molecular generation and optimization. As illustrated in \Cref{fig:boltz_as_fm}, we extract atom-level representations from Boltz for a given small molecule and evaluate their expressiveness across a broad range of small-molecule downstream tasks via probing and distillation. 


%We show that Boltz provides strong atom-level representations out of the box, beyond its original protein–ligand co-folding objective. Through systematic experiments, we identify three key findings:
%\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
%\item \textbf{Competitive supervised learning (\Cref{sec:admet})}: On the extensive TDC ADMET benchmark, Boltz representations match or outperform representations from specialized small-molecule representations like the ones from MiniMol and MolGPS.

%\item \textbf{Accelerated generative modeling (\Cref{sec:mol_gen}):} Leveraging the representation alignment~\citep{yu2024representation}, we show that distilling Boltz representations into molecular generative models improves molecular generation quality.

%\item \textbf{Structure-guided ligand discovery (\Cref{sec:structure_guided}):} We show that Boltz representations enhance optimization in structure-based ligand design, providing a stronger learning signal that improves sample efficiency.
%\end{itemize}
%These findings suggest that the representational capacity of cutting-edge protein models has been underexplored by the community, and position Boltz as a strong baseline for small-molecule foundation models. We also note the {complementarity of Boltz representations} with existing foundation models, and the improvement in downstream performance from the {use of protein context} (\Cref{sec:discussion}).

%Beyond empirical evaluations of Boltz representations, we also provide three actionable insights for the molecular machine learning community:
%\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
%\item \textbf{Co-folding as pretraining.} We show that predicting 3D protein-ligand interactions provides effective supervision for atom-level molecular representation learning. This also complements existing property-specific pretraining pipelines by yielding distinct representation spaces.
%\item \textbf{Representation-guided molecular optimization.} We extend representation alignment to online reinforcement learning for molecular discovery, showing that dense representation-level auxiliary supervision improves sample efficiency beyond scalar rewards alone.
%\item \textbf{Complementary representation ensembling.} We show that combining representations with low alignment, e.g., Boltz2 ensembled with MolE \citep{mendez2024mole}, outperforms higher alignment combinations, e.g., Boltz2 ensembled with MiniMol \citep{klaser2024minimol}, providing a useful strategy for representation fusion.
%\end{itemize}

==> 1_intro_V2.tex <==
\section{Introduction}

Large-scale representation learning has shown strong transferability across a wide range of downstream tasks, particularly in language~\citep{llama3, gpt4} and vision domains~\citep{vit, dinov2}. Foundation models with large-scale pretraining have become essential for achieving state-of-the-art performance in downstream applications, serving as powerful feature extractors~\citep{radford2021learning} for predictive tasks. Beyond predictive tasks, researchers have leveraged their representations to enhance generative modeling, including distillation into denoising models~\citep{yu2024representation} and use as latent embeddings for latent diffusion models~\citep{rae}. 

In the small-molecule domain, this paradigm has motivated foundation models that learn transferable atom-level representations for drug discovery tasks such as ADMET prediction~\citep{huang2021therapeutics}. Most existing models learn from molecules considered in isolation: each training example is a small molecule associated with molecule-level supervision such as bioassay labels and quantum-chemical properties~\citep{mendez2024mole,klaser2024minimol,kim2024quantum,zhou2023unimol,li2023knowledge,sypetkowski2024scalability}. Although these models differ in architecture and objective, they share a common design choice: the small molecule itself is the primary object of representation learning, without explicit modeling of an interacting molecular partner.

%Similarly, researchers in the small-molecule domain have explored foundation models to obtain transferable molecular representations, which is significant to solve a range of downstream tasks for drug discovery, e.g., ADMET prediction~\citep{huang2021therapeutics}. Especially, existing studies have focused on atom-level representation learning for small molecules, aiming to encode atom-level mechanisms through pretraining objectives such as masked token prediction, bioassay supervision, quantum property regression, and 3D structure prediction ~\citep{mendez2024mole,klaser2024minimol,kim2024quantum,zhou2023unimol,li2023knowledge,sypetkowski2024scalability}. Although these models differ in architecture and objective, they share a common paradigm: they learn molecular representations from molecules in isolation.

%These models differ in architecture and objective, but share a common paradigm: \textit{they learn molecular representations from standalone molecular data}. 
%However, in vision and natural language processing, strong representations are often learned by going beyond standalone data and incorporating complementary cross-modal or relational supervision \citep{radford2021learning,jia2021scaling,zhai2022lit}. The molecular domain likewise provides an analogous source of supervision through extensively accumulated high-quality inter-molecular interaction data: \textit{protein-ligand co-folding 3D structure} \citep{burley2021rcsb}, where a small molecule interacts with a protein to form a protein-ligand complex. This motivates a new question:
This is in contrast to vision and language, where strong representations often arise from supervision beyond standalone data, such as cross-modal or relational signals~\citep{radford2021learning,jia2021scaling,zhai2022lit}. We argue that the molecular domain has an analogous but underexplored source of such supervision: protein-ligand co-folding structures~\citep{burley2021rcsb}, in which a small molecule interacts with a protein at the atomic level.

We hypothesize that learning protein-ligand interactions provides richer supervision than learning from standalone molecular data alone, as it captures the atom-level mechanisms underlying interactions in bound conformations, including hydrogen bonding and electrostatic interactions. If this holds, protein-ligand complexes would constitute a new supervision source for molecular representation learning, complementary to the standalone molecular data. We therefore ask:
\begin{center}
\noindent\fcolorbox{black}{gray!15}{
\parbox{0.92\linewidth}{
\centering
\textit{Can protein-ligand co-folding models provide strong atom-level representations for standalone small-molecule tasks?}
}
}
\end{center}
Timely, modern protein–ligand co-folding models have transitioned from residue-level to atom-level modeling. AlphaFold3~\citep{abramson2024accurate} and its open-weight counterpart Boltz~\citep{wohlwend2024boltz1,passaro2025boltz2} are trained on large collections of protein-ligand complexes and learns atomistic representations to predict protein-ligand complexes with full atomic detail. Although their purpose is structure prediction, we can transfer their atomistic representations to standalone small-molecule tasks. %We therefore ask:

Although repurposing protein–ligand co-folding models for small-molecule representation learning is conceptually straightforward, it has not been systematically studied. This gap is important because the broader utility of co-folding models remains debated: recent studies suggest that models such as AlphaFold3 may rely heavily on MSA-derived evolutionary patterns rather than a genuine atom-level understanding of molecular interactions \citep{stahl2023protein,brotzakis2025alphafold}. Establishing this baseline therefore allows us to test whether the interaction-aware supervision learned by modern co-folding models transfers beyond their original structure-prediction objective.


\input{resource/background_figure}


\textbf{Contribution.} In this work, we investigate the potential of co-folding model, Boltz2, as a source of representations for small-molecule tasks, bridging cutting-edge protein-centric models and atom-level representation learning for small molecules. As illustrated in \Cref{fig:boltz_as_fm}, we extract atom-level representations from Boltz2 for a given small molecule and evaluate their expressiveness across a broad range of small-molecule downstream tasks. Notably, our work is the first to show that informative molecular representations can improve molecular generation and optimization.

%We show that Boltz2 provides strong atom-level representations out of the box, beyond its original protein–ligand co-folding objective. 
Through systematic experiments, we identify four key findings that position modern co-folding model, in particular Boltz2, as a strong baseline for small-molecule foundation models.
\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
\item \textbf{Predictive transfer (\Cref{sec:admet})}: Boltz representations match or outperform specialized small molecular foundation models on the extensive TDC ADMET benchmark.
\item \textbf{Generative transfer (\Cref{sec:mol_gen}):} Boltz2 representations improve molecular generative models with representation alignment-based distillation~\citep{yu2024representation}.
\item \textbf{Optimization transfer (\Cref{sec:structure_guided}):} Boltz2 representations enhance sample efficiency for designing ligands to maximize the Boltz2's binding affinity score using a new distillation method. 
%\item \textcolor{blue}{\textbf{Representation complementarity (\Cref{sec:ablation}):} Co-folding representations occupy a distinct representation space from models pretrained on standalone molecular data.}
\item \textbf{Representation analysis (\Cref{sec:ablation}):} Boltz2 yields representation space complementing existing molecular models; further analyses cover protein context and layer-wise behavior.
\end{itemize}
%These findings suggest that the representational capacity of co-folding-based representation learning has been underexplored by the community. position modern co-folding model, Boltz2, as a strong baseline for small-molecule foundation models. 
%We also note the \textit{complementarity of Boltz2 representations} with existing foundation models trained on standalone molecular data, and the improvement in downstream performance from the \textit{use of protein context} (\Cref{sec:ablation}).
Finally, we provide actionable insights for the molecular machine learning community. First, we extend representation alignment to online reinforcement learning for molecular discovery, showing how dense signals from the reward model can be used to improve sample efficiency beyond scalar rewards alone. Second, we show that combining weakly aligned representations, e.g., Boltz2 with MolE \citep{mendez2024mole}, outperforms more strongly aligned combinations, e.g., Boltz2 with MiniMol \citep{klaser2024minimol}, suggesting a practical strategy for representation fusion. 



==> 1_intro_V3.tex <==
\section{Introduction}

Large-scale representation learning has shown strong transferability across a wide range of downstream tasks, particularly in language~\citep{llama3, gpt4} and vision domains~\citep{vit, dinov2}. Foundation models with large-scale pretraining have become essential for achieving state-of-the-art performance in downstream applications, serving as powerful feature extractors~\citep{radford2021learning} for predictive tasks. Beyond predictive tasks, researchers have leveraged their representations to enhance generative modeling, including distillation into denoising models~\citep{yu2024representation} and use as latent embeddings for latent diffusion models~\citep{rae}. 

In the small-molecule domain, this paradigm has motivated foundation models that learn transferable atom-level representations for drug discovery tasks such as ADMET prediction~\citep{huang2021therapeutics}. Most existing models learn from molecules considered in isolation: each training example is a small molecule associated with molecule-level supervision such as bioassay labels and quantum-chemical properties~\citep{mendez2024mole,klaser2024minimol,kim2024quantum,zhou2023unimol,li2023knowledge,sypetkowski2024scalability}. Although these models differ in architecture and objective, they share a common design choice: the small molecule itself is the primary object of representation learning, without explicit modeling of an interacting molecular partner.

This is in contrast to vision and language, where strong representations often arise from supervision beyond standalone data, such as cross-modal or relational signals~\citep{radford2021learning,jia2021scaling,zhai2022lit}. We argue that the molecular domain has an analogous but underexplored source of such supervision: protein-ligand co-folding structures~\citep{burley2021rcsb}, in which a small molecule interacts with a protein. We ask:
\begin{center}
\noindent\fcolorbox{black}{gray!15}{
\parbox{0.92\linewidth}{
\centering
\textit{Can protein-ligand co-folding models provide strong atom-level representations for standalone small-molecule tasks?}
}
}
\end{center}
We hypothesize that learning protein-ligand interactions provides richer supervision than learning from standalone molecular data alone, as it captures the atom-level mechanisms underlying interactions in bound conformations, including hydrogen bonding and electrostatic interactions. If this holds, protein-ligand complexes would constitute a new supervision source for molecular representation learning, complementary to the standalone molecular data. 

Timely, modern protein-ligand co-folding models have transitioned from residue-level to atom-level modeling. AlphaFold3~\citep{abramson2024accurate} and its open-weight counterpart Boltz~\citep{wohlwend2024boltz1,passaro2025boltz2} are trained on large collections of protein-ligand complexes and learns atomistic representations to predict protein-ligand complexes with full atomic detail. Although their purpose is structure prediction, we can transfer their atomistic representations to standalone small-molecule tasks. 

Although repurposing protein-ligand co-folding models for small-molecule representation learning is conceptually straightforward, it has not been systematically studied. This gap is important because the broader utility of co-folding models remains debated: recent studies suggest that models such as AlphaFold3 may rely heavily on MSA-derived evolutionary patterns rather than a genuine atom-level understanding of molecular interactions \citep{stahl2023protein,brotzakis2025alphafold}. Establishing this baseline therefore allows us to test whether the interaction-aware supervision learned by modern co-folding models transfers beyond their original structure-prediction objective.


\input{resource/background_figure}


\textbf{Contribution.} In this work, we investigate the potential of co-folding model, Boltz2, as a source of representations for small-molecule tasks, bridging cutting-edge protein-centric models and atom-level representation learning for small molecules. As illustrated in \Cref{fig:boltz_as_fm}, we extract atom-level representations from Boltz2 for a given small molecule and evaluate their expressiveness across a broad range of small-molecule downstream tasks. Notably, our work is the first to show that informative molecular representations can improve molecular generation and optimization.

%We show that Boltz2 provides strong atom-level representations out of the box, beyond its original protein-ligand co-folding objective. 
Through systematic experiments, we identify four key findings that position modern co-folding model, in particular Boltz2, as a strong baseline for small-molecule foundation models.
\begin{itemize}[topsep=-1.0pt,itemsep=1.0pt,leftmargin=3.5mm]
\item \textbf{Predictive transfer (\Cref{sec:admet})}: Boltz representations match or outperform specialized small molecular foundation models on the extensive TDC ADMET benchmark.
\item \textbf{Generative transfer (\Cref{sec:mol_gen}):} Boltz2 representations improve molecular generative models with representation alignment-based distillation~\citep{yu2024representation}.
\item \textbf{Optimization transfer (\Cref{sec:structure_guided}):} Boltz2 representations enhance sample efficiency for designing ligands to maximize the Boltz2's binding affinity score using a new distillation method. 
%\item \textcolor{blue}{\textbf{Representation complementarity (\Cref{sec:ablation}):} Co-folding representations occupy a distinct representation space from models pretrained on standalone molecular data.}
\item \textbf{Representation analysis (\Cref{sec:ablation}):} Boltz2 yields representation space complementing existing molecular models; further analyses cover protein context and layer-wise behavior.
\end{itemize}
%These findings suggest that the representational capacity of co-folding-based representation learning has been underexplored by the community. position modern co-folding model, Boltz2, as a strong baseline for small-molecule foundation models. 
%We also note the \textit{complementarity of Boltz2 representations} with existing foundation models trained on standalone molecular data, and the improvement in downstream performance from the \textit{use of protein context} (\Cref{sec:ablation}).
Finally, we provide actionable insights for the molecular machine learning community. First, we extend representation alignment to online reinforcement learning for molecular discovery, showing how dense signals from the reward model can be used to improve sample efficiency beyond scalar rewards alone. Second, we show that combining weakly aligned representations, e.g., Boltz2 with MolE \citep{mendez2024mole}, outperforms more strongly aligned combinations, e.g., Boltz2 with MiniMol \citep{klaser2024minimol}, suggesting a practical strategy for representation fusion. 



==> 2_related_work.tex <==
\section{Background}

\textbf{Boltz.}

\textbf{Foundation models for molecules.}

\textbf{Representation alignment.}

==> 3_method.tex <==
\section{Methods}\label{sec:method}


\subsection{ADMET property prediction}\label{sec:admet_methods}

\textbf{Datasets.} We conduct experiments on the Therapeutics Data Commons (TDC) ADMET benchmark datasets~\citep{huang2021therapeutics}, which consist of 22 ADMET property prediction tasks for small molecules represented as SMILES strings~\citep{weininger1988smiles}. We follow the standard data splits, evaluation metrics, and five random seeds. Detailed benchmark settings are provided in Supplementary Table~\ref{tab:admet_stats_metrics}.

\textbf{Representation extraction and probing.} We apply linear probing to Boltz2 molecular representations for property prediction. Atom-wise pair representations are extracted from the Boltz2 Pairformer trunk by concatenating outputs from multiple layers. The pooled representation is fed into a multi-layer perceptron (MLP) for target label prediction. Full details on the pooling strategy and probing network architecture are provided in Supplementary Section~\ref{supp:admet_details}.

%\textbf{Baselines.} We consider two deep learning-based methods, DeepAutoQSAR~\citep{dixon2016autoqsar} and DeepPurpose~\citep{huang2020deeppurpose}. We also consider six foundation models specialized for ADMET property prediction: KPGT~\citep{li2023knowledge}, UniQSAR~\citep{gao2023uniqsarautomltoolmolecular}, MolE~\citep{mendez2024mole}, MiniMol~\citep{klaser2024minimol}, QIP~\citep{kim2024quantum}, and MolGPS~\citep{sypetkowski2024scalability}. Among these, MolGPS and UniQSAR employ ensemble-based approaches. For a direct comparison, we combine Boltz2 representations with those from MiniMol (Boltz2$^\text{Mini.}$).


\subsection{Molecular generation}\label{sec:mol_gen_methods}

\textbf{Datasets.} We conduct molecular generation experiments on the widely used ZINC250k dataset~\citep{jo2022score,vignac2022digress,jangsimple,kong2023autoregressive,jo2023graph,seo2025learning}. We train generative models on this dataset and evaluate their performance on $10{,}000$ generated molecules following prior work.

\textbf{Representation alignment.} We adopt a representation alignment-based distillation \citep{yu2024representation} to existing diffusion-based molecular generative models, specifically GruM~\citep{jo2023graph}. We parameterize the denoising model of GruM with a four-layer Pairformer that outputs single and pair representations as hidden representations for denoising atom and bond types, respectively.

We distill Boltz2 representations into GruM via representation alignment by training the denoising model to maximize the cosine similarity between its hidden representations of noisy molecules and the corresponding Boltz2 representations of clean molecules. We apply the alignment loss at the middle layer of the denoising model, aligning its single and pair representations with Boltz single and pair representations. Details are provided in Supplementary Section~\ref{supp:mol_gen_details}.

\textbf{CKNNA metric.} We measure representation alignment using Centered Kernel Nearest-Neighbor Alignment (CKNNA)~\citep{huh2024platonic}, which evaluates local alignment between two representation spaces based on shared nearest-neighbor structure (Supplementary Section~\ref{supp:cknna}).


\subsection{Structure-guided ligand discovery}\label{sec:structure_methods}

\textbf{Target proteins.} We use seven target proteins as benchmarks. First, we consider four benchmark targets from the Boltz2 paper, where Boltz2 shows strong binding affinity prediction performance~\citep{passaro2025boltz2}: TYK2, CDK2, JNK1, and P38. We additionally include three proteins from distinct classes: CA2 as a metalloenzyme, THROMBIN as a serine protease, and FABP4 as a lipid-binding protein, covering diverse protein domains and ligand interaction mechanisms.

\textbf{SynFlowNet-Boltz pipeline.} We use the SynFlowNet-Boltz pipeline introduced in the Boltz2 paper~\citep{passaro2025boltz2} for online ligand discovery. The SynFlowNet policy sequentially selects synthetic actions to build ligand molecules, and Boltz2 computes binding affinity scores as rewards to update the policy. For each generated terminal molecule $m$, the reward is computed as:
\begin{equation*}
r=\text{max}\Big(\frac{-\text{affinity}+2}{4},0\Big)\cdot\text{likelihood},
\end{equation*}
where $\text{affinity}$ is the Boltz2-predicted binding affinity score and $\text{likelihood}$ denotes the Boltz2-predicted likelihood of binding to the corresponding binding site.

\textbf{Representation alignment.} In our experiments, we extend SynFlowNet-Boltz setup by incorporating representation alignment-based distillation into the policy. Specifically, we maximize the cosine similarity between the policy’s second-layer single representations and corresponding Boltz2 single representations. Note that representations are aligned on ligand molecules, using Boltz2 ligand representations that are obtained as a byproduct of the Boltz2 binding affinity computation. The overall implementation and hyperparameters follow prior settings \citep{passaro2025boltz2}, with details provided in Supplementary Section~\ref{supp:synflownet_details}.

\textbf{Metrics.} First, we measure the number of high-score molecules discovered as a function of reward evaluations during online training, reflecting sample efficiency. A molecule is considered high-reward if its Boltz2 screening score~\citep{passaro2025boltz2} exceeds $0.75$ (or $1.2$ for CA2, to account for metal coordination effects). Second, we measure the number of modes, defined as the number of distinct high-scoring molecules with pairwise Tanimoto similarity below $0.6$.


==> 4_discussion.tex <==
%\section{Discussion}\label{sec:discussion}



%An intriguing observation across our experiments is that Boltz2 exhibits relatively low average CKNNA alignment with existing molecular foundation models, despite consistently outperforming them on downstream predictive, generative, and structure-guided tasks. This suggests that Boltz2 does not improve performance by refining or better approximating representations learned by prior molecular models. Instead, it appears to capture a qualitatively different set of features.

%We hypothesize that this discrepancy stems from the nature of Boltz2’s pretraining objective. Unlike small-molecule foundation models that primarily focus on intrinsic molecular properties or graph-level chemical patterns, Boltz2 is trained to predict atomic-resolution protein–ligand interactions in three-dimensional space. This objective directly supervises intermolecular geometry, spatial complementarity, and interaction-specific constraints, which may be weakly represented or entirely absent in property-centric molecular pretraining.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately reflect the paper’s contribution and scope: identifying protein-ligand co-folding as an underexplored source of supervision for small-molecule representation learning and evaluating Boltz2 as an off-the-shelf representation model. The paper also clearly scopes the validation to ADMET prediction, molecular generation, structure-guided ligand optimization, and representation complementarity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of the work in \Cref{sec:discussion}. In summary, 3D supervision has limitations in understanding complete atomistic mechanisms. We also restrict our study to conventional frozen-backbone setting, leaving full backbone fine-tuning.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not address theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the detailed experimental settings in \Cref{supp:synflownet_details,supp:mol_gen_details,supp:molopt_details}. We provide our code as mentioned in \Cref{supp:avail_code}.%\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide our code as mentioned in \Cref{supp:avail_code}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the detailed hyper-parameters in \Cref{supp:synflownet_details,supp:mol_gen_details,supp:molopt_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report standard deviations in \Cref{tab:admet_stats_metrics,tab:full_gen}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We mention the use of NVIDIA B200 GPUs in \Cref{supp:molopt_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Our work conforms NeurIPS Code of Ethics, including the anonymity of the authors.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed the positive and negative social impacts in last of Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cited the original paper that produced the code package or dataset in \Cref{supp:avail_code}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please refer the references. We also refer Boltz2 under MIT license at \Cref{supp:avail_code}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not release any new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include crowsourcing experiments and research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve any crowdsourcing or research with human objects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We used AI-based writing assistants to improve the grammar. These tools were used only for editorial improvements. The technical content, methodology, and experimental results were entirely authored by the researchers.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> resource/boltz_mole_meta_table.tex <==
\begin{wrapfigure}{r}{0.5\linewidth}
\caption{\textbf{Combining Boltz2 representations with complementary representations.} Combining Boltz2 representations with complementary representations (MolE; see \Cref{fig:cknna}) significantly improves performance on some benchmarks compared to combinations with more highly aligned representations (MiniMol).}
\label{tab:boltz_mole_meta}
\centering
\scalebox{0.86}{\centering
\begin{tabular}{l c c c}
\toprule
\textbf{Model} & CYP2C9 V. & CYP2D6 V. & CYP3A4 V. \\
\midrule
\textbf{MolE} & 0.80 & 0.68 & 0.87 \\ 
\textbf{Mini.} & 0.82 & 0.72 & 0.88 \\
\midrule
\textbf{Boltz2} & 0.82 & 0.69 & 0.85 \\
\textbf{Boltz2}$^{\mathrm{MolE}}$ & \textbf{0.88{\scriptsize (+.06)}} & \textbf{0.77{\scriptsize (+.08)}} & \textbf{0.89{\scriptsize (+.04)}} \\
\textbf{Boltz2}$^{\mathrm{Mini.}}$ & 0.86{\scriptsize (+.04)} & 0.72{\scriptsize (+.03)} & 0.88{\scriptsize (+.03)} \\
\bottomrule
\end{tabular}}
\vspace{-.1in}
\end{wrapfigure}


==> resource/gen_sota_table.tex <==
\begin{wraptable}{r}{0.46\textwidth}
\centering
\vspace{-1.0em}
\caption{\textbf{Comparison with post-2024 SOTA baselines on ZINC250k.} Boltz2-based distillation yields \textbf{best} performance.}
\label{tab:zinc_short}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c c}
\toprule
\textbf{Method} & \textbf{Valid $\uparrow$} & \textbf{FCD $\downarrow$} & \textbf{NSPDK $\downarrow$} \\
\midrule
GruM   & 98.65 & 2.26 & 0.0015 \\
GVT    & 99.57 & \textbf{1.16} & 0.0689 \\
GBD    & 97.87 & 2.25 & 0.0018 \\
DeFoG  & 99.22 & 1.42 & 0.0008 \\
TopBF  & 99.37 & 1.39 & 0.0008 \\
SID    & 99.50 & 2.01 & 0.0021 \\
\midrule
\rowcolor{aliceblue!60}
\textbf{Boltz2} & \textbf{99.65} & 1.31 & \textbf{0.0005} \\
\bottomrule
\end{tabular}
\vspace{-1.0em}
\end{wraptable}

==> resource/tab_unimol.tex <==
\begin{wraptable}{r}{0.35\linewidth}
\centering
\vspace{-.2in}
\caption{\textbf{Boltz2 vs.\ UniMol2 (1B).} \textbf{Bold} indicates the best. The results indicate that the performance of Boltz2 stems from co-folding.}
\label{tab:boltz_vs_unimol2_1b}
\small
\scalebox{0.86}{
\begin{tabular}{l c c}
\toprule
\textbf{Dataset} & \textbf{Boltz2} & \textbf{UniMol2} \\
\midrule
Caco2 $\downarrow$         & \textbf{0.30} & 0.41 \\
HIA $\uparrow$             & \textbf{0.99} & 0.87 \\
Pgp $\uparrow$             & \textbf{0.93} & 0.90 \\
Bioavailability $\uparrow$ & \textbf{0.75} & 0.64 \\
Lipophilicity $\downarrow$ & \textbf{0.45} & 0.61 \\
Solubility $\downarrow$    & \textbf{0.66} & 0.81 \\
\hline
BBB $\uparrow$             & \textbf{0.93} & 0.86 \\
PPBR $\downarrow$          & \textbf{7.65} & 8.95 \\
VDss $\uparrow$            & \textbf{0.74} & 0.70 \\
\hline
CYP2C9 V.\ $\uparrow$      & \textbf{0.82} & 0.77 \\
CYP2D6 V.\ $\uparrow$      & \textbf{0.69} & 0.62 \\
CYP3A4 V.\ $\uparrow$      & \textbf{0.85} & 0.81 \\
CYP2C9 S.\ $\uparrow$      & \textbf{0.36} & 0.33 \\
CYP2D6 S.\ $\uparrow$      & \textbf{0.52} & 0.44 \\
CYP3A4 S.\ $\uparrow$      & \textbf{0.62} & 0.58 \\
\hline
Half Life $\uparrow$       & \textbf{0.62} & 0.48 \\
Clearance H.\ $\uparrow$   & \textbf{0.62} & 0.45 \\
Clearance M.\ $\uparrow$   & 0.61 & \textbf{0.62} \\
\hline
LD50 $\downarrow$          & \textbf{0.40} & 0.50 \\
hERG $\uparrow$            & \textbf{0.86} & 0.75 \\
AMES $\uparrow$            & \textbf{0.91} & 0.88 \\
DILI $\uparrow$            & \textbf{0.89} & 0.83 \\
\bottomrule
\end{tabular}}
\vspace{-.1in}
\end{wraptable}
